Multivariate Functional Principal Component Analysis for Data Observed on Different (Dimensional) Domains

Existing approaches for multivariate functional principal component analysis are restricted to data on the same one-dimensional interval. The presented approach focuses on multivariate functional data on different domains that may differ in dimension, e.g. functions and images. The theoretical basis for multivariate functional principal component analysis is given in terms of a Karhunen-Lo\`eve Theorem. For the practically relevant case of a finite Karhunen-Lo\`eve representation, a relationship between univariate and multivariate functional principal component analysis is established. This offers an estimation strategy to calculate multivariate functional principal components and scores based on their univariate counterparts. For the resulting estimators, asymptotic results are derived. The approach can be extended to finite univariate expansions in general, not necessarily orthonormal bases. It is also applicable for sparse functional data or data with measurement error. A flexible R-implementation is available on CRAN. The new method is shown to be competitive to existing approaches for data observed on a common one-dimensional domain. The motivating application is a neuroimaging study, where the goal is to explore how longitudinal trajectories of a neuropsychological test score covary with FDG-PET brain scans at baseline. Supplementary material, including detailed proofs, additional simulation results and software is available online.

==> chapterShort/sketchProof.tex <==
\section*{Appendix: Proof  for Proposition~\ref{prop:multi_single_EV}, Part 2}


Assume the functional covariates $X^{(1)} , \ldots ,  X^{(p)}$ do each have a finite Karhunen-Lo\`{e}ve representation, i.e. for each $j = 1, \ldots, p: ~X^{(j)} = \sum \nolimits _{m = 1}^{M_j} \xi_m^{(j)} \phi_m^{(j)}$. Let $\Gamma \psi = \nu \psi$. Then for all $j = 1 , \ldots ,  p$ and $t_j \in \mathcal{T}_j$
\begin{align*}
\left( \Gamma \psi \right)^{(j)}(t_j)  
&= \sum \nolimits _{k=1}^p \int_{\mathcal{T}_k} \operatorname{Cov} \left(X^{(k)}(s_k), X^{(j)}(t_j) \right) \psi ^{(k)}(s_k) \mathrm{d}  s_k \\
&= \sum \nolimits _{k=1}^p  \sum \nolimits _{l = 1}^{M_j} \sum \nolimits _{n = 1}^{M_k}   \underbrace{\operatorname{Cov} \left( \xi_l^{(j)}, \xi_n^{(k)} \right)}_{=: Z_{ln}^{(jk)}}  \phi_l^{(j)}(t_j)   \underbrace{\int_{\mathcal{T}_k}  \phi_n^{(k)}(s_k)  \psi ^{(k)}(s_k) \mathrm{d}  s_k}_{=: c_n^{(k)}} 
\stackrel{!}{=} \nu \psi ^{(j)}(t_j).
\end{align*}
With a similar argumentation as in \citet[Chapter 1.3.]{Zemyan:2012} it holds
\begin{align}
& \sum \nolimits _{k=1}^p  \sum \nolimits _{l = 1}^{M_j}  \sum \nolimits _{n = 1}^{M_k}  Z_{ln}^{(jk)}  \phi_l^{(j)}(t_j)  c_n^{(k)} = \nu \psi ^{(j)}(t_j) \label{eq:eVecsMulti}\\
\Rightarrow &
\int_{\mathcal{T}_j} \phi_m^{(j)}(t_j) \cdot \sum \nolimits _{k=1}^p \sum \nolimits _{l = 1}^{M_j}  \sum \nolimits _{n = 1}^{M_k}   Z_{ln}^{(jk)}  \phi_l^{(j)}(t_j)  c_n^{(k)} \mathrm{d}  t_j = \int_{\mathcal{T}_j} \phi_m^{(j)}(t_j) \cdot \nu \psi ^{(j)}(t_j) \mathrm{d}  t_j \nonumber \\
\Leftrightarrow &
\sum \nolimits _{k=1}^p  \sum \nolimits _{n = 1}^{M_k}   Z_{mn}^{(jk)}  c_n^{(k)} = \nu c_m^{(j)}  \nonumber
\end{align}
for $m \in \{1 , \ldots ,  M_j\}$ due to orthonormality of $\phi_m^{(j)}$.  Since $m$ and $j$  were arbitrarily chosen, this is equivalent to 
\[
\underbrace{
\begin{pmatrix}
\boldsymbol{Z^{(11)} }& \ldots  & \boldsymbol{Z^{(1p)}} \\
\vdots& \ddots & \vdots \\
\boldsymbol{Z^{(p1)}}& \ldots & \boldsymbol{Z^{(pp)}}
\end{pmatrix}
}_{=:\boldsymbol{Z}}
\underbrace{
\begin{pmatrix}
\boldsymbol{c^{(1)}} \\
\vdots \\
\boldsymbol{c^{(p)}}
\end{pmatrix}}_{=:\boldsymbol{c}}
=
\nu
\begin{pmatrix}
\boldsymbol{c^{(1)}} \\
\vdots \\
\boldsymbol{c^{(p)}}
\end{pmatrix}
\] 
with matrices $\boldsymbol{Z^{(jk)}} \in \mathbb R ^{M_j \times M_k}$ and $\boldsymbol{c^{(j)}} \in \mathbb R ^{M_j}$. The last equation is again an eigenequation for the symmetric (and since $\nu \geq 0$) positive semidefinite block matrix $\boldsymbol{Z} \in \mathbb R ^{M_+ \times M_+}$.
Let $\nu_1 \geq \ldots \geq \nu_M > 0,~ M \leq M_+$ be the non-zero eigenvalues of $\boldsymbol{Z}$. These are also the only non-zero eigenvalues of $\Gamma$ and the elements $\psi_m^{(j)}$ of the associated eigenfunctions $\psi_m$ are parametrized by the (orthonormal) eigenvectors $\boldsymbol{c_1} , \ldots ,  \boldsymbol{c_M}$ associated with $\nu_1 , \ldots ,  \nu_M$:
\[
 \psi_m^{(j)}(t_j)
\stackrel{\eqref{eq:eVecsMulti}}{=} \frac{1}{\nu_m}
\sum \nolimits _{k=1}^p  \sum \nolimits _{l = 1}^{M_j} \sum \nolimits _{n = 1}^{M_k}   Z_{ln}^{(jk)}   [\boldsymbol{c_m}]^{(k)}_n  \phi_l^{(j)}(t_j) 
= \sum \nolimits _{l = 1}^{M_j} [\boldsymbol{c_m}]_l^{(j)} \phi_l^{(j)}(t_j), \quad t_j \in \mathcal{T}_j
\]
for $m = 1 , \ldots ,  M,~ j = 1 , \ldots ,  p.$ The eigenfunctions form an orthonormal system with respect to $\myscal{\cdot}{\cdot}$:
\[
\myscal{\psi_m}{\psi_n}
= \sum \nolimits _{j = 1}^p \scal{\psi_m^{(j)}}{\psi_n^{(j)}} 
= \sum \nolimits _{j = 1}^p \sum \nolimits _{l = 1}^{M_j} [\boldsymbol{c_m}]^{(j)}_{l} [\boldsymbol{c_n}]^{(j)}_{l}  
= \boldsymbol{c_n} ^\top  \boldsymbol{c_m} = \delta_{mn}.
\]
The Karhunen-Lo\`{e}ve decomposition of $X$ is hence given by $X = \sum \nolimits  _{m=1}^M \rho_m \psi_m$ with scores
\[
\rho_m
 = \myscal{X}{\psi_m} 
= \sum \nolimits _{j = 1}^p \sum \nolimits _{n = 1}^{M_j}\left[\boldsymbol{c_m}\right]_n^{(j)}  \xi_n^{(j)}
\]
and $\mathbb{E}(\rho_m)=0,~\operatorname{Cov}(\rho_m, \rho_n) = \nu_m \delta_{mn},~ m = 1 , \ldots ,  M \leq M_+$.

